A Practical and Worst-Case Efficient Algorithm for Divisor Methods of Apportionment

Proportional apportionment is the problem of assigning seats to parties according to their relative share of votes. Divisor methods are the de-facto standard solution, used in many countries. In recent literature, there are two algorithms that implement divisor methods: one by Cheng and Eppstein (ISAAC, 2014) has worst-case optimal running time but is complex, while the other (Pukelsheim, 2014) is relatively simple and fast in practice but does not offer worst-case guarantees. We demonstrate that the former algorithm is much slower than the other in practice and propose a novel algorithm that avoids the shortcomings of both. We investigate the running-time behavior of the three contenders in order to determine which is most useful in practice.

==> app-commands.tex <==
\makeatletter


	\theoremstyle{break}
	\ifarxiv[%
		\theorempreskip{2\topsep}
	]%
	{%
		\theorempreskipamount2\topsep
	}
	\newtheorem{theorem}{Theorem}%[section]
	
	
	\theoremstyle{plain}
	\ifarxiv[%
		\theorempreskip{\topsep}
	]{%
		\theorempreskipamount\topsep
	}
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{conjecture}[theorem]{Conjecture}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{definition}[theorem]{Definition}
	
	\theoremstyle{plain}
	\theorembodyfont{\upshape}
	\newtheorem{property}[theorem]{Property}
	\newtheorem{fact}[theorem]{Fact}
	\theorembodyfont{\upshape}
	\newtheorem{algorithm}{Algorithm}
	\newtheorem{problem}{Problem}
	\theorembodyfont{\upshape\small}
	\newtheorem{example}[theorem]{Example}
	\def\continuedexref{ex:dummyref}
	\newtheorem*{examplecontinued}{\wref{\continuedexref}\space Continued}
	
	\newenvironment{examplectd}[1]
	  {\def\continuedexref{#1}\examplecontinued}
	  {\endexamplecontinued}
	
	\theorembodyfont{\upshape}
	\theoremsymbol{\raisebox{-.15ex}{$\Box$}}
	\qedsymbol{\raisebox{-.15ex}{$\Box$}}
	\theoremstyle{proofstyle}
	\newtheorem{proof}{Proof}



\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}


\newcommand{\Oh}{\ensuremath{O}\xspace}
\newcommand{\oh}{\ensuremath{o}\xspace}
\newcommand{\Th}{\ensuremath{\Theta}\xspace}
\newcommand{\Om}{\ensuremath{\Omega}\xspace}
\newcommand{\om}{\ensuremath{\omega}\xspace}

\newcommand\harm[1]{\ensuremath{H_{#1}}}

\newcommand{\vect}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\mset}[1]{\mathcal{#1}}

\newcommand\pe{\phantom{{}={}}}
\newcommand\ppe{\phantom{=}}
\newcommand\ce{\colonequals}

\newcommand\rel[1]{\mathrel{\:{#1}\:}}
\newcommand\wrel[1]{\mathrel{\;{#1}\;}}
\newcommand\wwrel[1]{\mathrel{\;\;{#1}\;\;}}
\newcommand\bin[1]{\mathbin{\:{#1}\:}}
\newcommand\wbin[1]{\mathbin{\;{#1}\;}}
\newcommand\wwbin[1]{\mathbin{\;\;{#1}\;\;}}

\newcommand{\eqwithref}[2][c]{%
	\relwithref[#1]{#2}{=}%
}
\newcommand{\relwithref}[3][c]{%
	\mathrel{\underset{\mathclap{\makebox[\widthof{$=$}][#1]{\scriptsize\wref{#2}}}}{#3}}%
}

\newcommand\tcases[4]{\ensuremath{%
	\bigl\{{\textstyle\scriptsize%
		\genfrac{}{}{0pt}{}{{#1}\hfill}{{#3}\hfill}\,%
		\genfrac{}{}{0pt}{}{{#2}\hfill}{{#4}\hfill}}%
}}

\newcommand\like[3][c]{\makeboxlike[#1]{\ensuremath{#2}}{\ensuremath{#3}}}

\newcommand{\highestavgsalgASCII}{IterativeMethod}
\newcommand\RWalgASCII{SandwichSelect}
\newcommand*{\CEalgASCII}{ChengEppsteinSelect}
\newcommand*{\PukalgASCII}{JumpAndStep}
\newcommand*\HAalg{\hyperref[alg:highest-averages]{\textsc{\highestavgsalgASCII}}\xspace}
\newcommand*\CEalg{\hyperref[alg:CE-main-procedure]{\textsc{\CEalgASCII}}\xspace}
\newcommand*\RWalg{\hyperref[alg:selection-algo-linear-candidates]{\textsc{\RWalgASCII}}\xspace}
\newcommand*\Pukalg{\hyperref[alg:jump-and-step]{\textsc{\PukalgASCII}}\xspace}
% Deprecated
\newcommand{\quadraticalgASCII}{SandwichSelectNaive}
\newcommand*\quadraticalg{\hyperref[alg:selection-algo-all-candidates]{\textsc{\quadraticalgASCII}}\xspace}


\newcommand{\appproblemascii}{Proportional Apportionment}
\newcommand*\appfunc{\ensuremath{f}\xspace}
\newcommand{\cutproblem}{\hyperref[prob:appproblem]{\textsf{\appproblemascii}}\xspace}

\newcommand*\drank{\ensuremath{\operatorname{index}_d}\xspace}

\newcommand{\algcomment}[1]{\quad\textsl{\small(#1)}}

\newenvironment{indented}{%
  \begin{adjustwidth}{2em}{2em}
}{%
  \end{adjustwidth}
}

\newcommand{\qqed}[1][]{% a dotted q.e.d. box that suggests an incomplete proof
  \ensuremath{\raisebox{-0.25ex}{%
    \tikz[baseline=0.0] %
    \draw[dash pattern=on 1.1pt off 1pt,line width=0.5pt] (0,0)         -- (0,.65em)
                                                          (0,.65em)     -- (.65em,.65em)
                                                          (.65em,.65em) -- (.65em,0)
                                                          (.65em,0)     -- (0,0);}_{\,#1}}}


%%%%% create an hbox of the given width height and depth
%%%%% beware, ugly TeX hack, may result in strange
%%%%% behavior
\def\makeboxwhd#1#2#3#4{\setbox0=\hbox{#4}%
\ht0=#2%
\dp0=#3%
\wd0=#1%
\box0%
}

%%%%% create an hbox of the size of #2, but insert #3
%%%%% #1 can be l, c or r and gives the horizontal position
\newdimen\makeboxdimen
%\setlength\fboxsep{-\fboxrule}
\newcommand\makeboxlike[3][l]{%
\setbox0=\hbox{#2}%
\global\makeboxdimen=\wd0%
\setbox1=\hbox{\makebox[\makeboxdimen][#1]{%
\makebox[0pt][#1]{#3}%
}}%
\ht1=\ht0%
\dp1=\dp0%
\box1%	
}

\newcommand\plaincenter[1]{%
	\mbox{}\hfill#1\hfill\mbox{}%
}


% Notation list
\def\mydots{\xleaders\hbox to.75em{\hfill.\hfill}\hfill}
\newlength\tmpLenNotations

\newenvironment{notations}[1][10em]{%
	\small
	\newcommand\notationentry[1]{%
		\settowidth\tmpLenNotations{##1}%
		\ifthenelse{\lengthtest{\tmpLenNotations > \labelwidth}}{%
			\parbox[b]{\labelwidth}{%
				\makebox[0pt][l]{##1}\\%
			}%
		}{%
			\mbox{##1}%
		}%
		\mydots\relax%
	}%
	\begin{list}{}{%
		\setlength\labelsep{0em}%
		\setlength\labelwidth{#1}%
		\setlength\leftmargin{\labelwidth+\labelsep+1em}%
		\renewcommand\makelabel{\notationentry}%
	}
	\newcommand\notation[1]{\item[{##1}]}
	\iflocal{%
		\renewcommand\notation[1]{\item[{##1}] \marginline{\tiny\texttt{\detokenize{##1}}}}
	}
	\raggedright
}{%
	\end{list}
}

\makeatother

